Molecular Diffusion Models with Virtual Receptors

Machine learning approaches to Structure-Based Drug Design (SBDD) have proven quite fertile over the last few years. In particular, diffusion-based approaches to SBDD have shown great promise. We present a technique which expands on this diffusion approach in two crucial ways. First, we address the size disparity between the drug molecule and the target/receptor, which makes learning more challenging and inference slower. We do so through the notion of a Virtual Receptor, which is a compressed version of the receptor; it is learned so as to preserve key aspects of the structural information of the original receptor, while respecting the relevant group equivariance. Second, we incorporate a protein language embedding used originally in the context of protein folding. We experimentally demonstrate the contributions of both the virtual receptors and the protein embeddings: in practice, they lead to both better performance, as well as significantly faster computations.

==> old/method_1.tex <==
%\todo{todo}{subsection}{Insert a highly rewritten version of Section 1 from our old overleaf.  It should introduce diffusion methods in general, and then specialize to the case of molecules, noting the importance of equivariance.}

\subsection{Diffusion Framework for Target-Aware Molecular Sampling}

We define $X^r = (x_{1}^{r},\cdots,x_{M}^{r})\in \mathcal{R}^{M\times 3}$ as the receptor point cloud with corresponding ordinal/categorical features  $H^r =(h_{1}^{r},\cdots,h_{M}^{r}) \in \mathcal{R}^{M\times f_m} $ and $X^l== (x_{1}^{l},\cdots,x_{N}^{l}) \in \mathcal{R}^{N\times 3}$ as the ligand  point cloud with corresponding ordinal/categorical features  $H^l =(h_{1}^{l},\cdots,h_{N}^{l}) \in \mathcal{R}^{N\times f_n}$

Diffusion models are a class of generative models that learn distribution by modelling the reverse diffusion processes e.g the denoising process. given a data point $x$ we define an Markov chain of latent variables $x_{1}\hdots x_{T} $ by progressively adding noise to the sample (diffusion process) that is defined by \cite{kingma2021variational} as the following:
\begin{equation}
    q(z_{t|x})=\mathcal{N}(z_(t)|\alpha_{t}x_{data},\sigma_{t}^{2}I)
\end{equation}
where $\alpha_{t} \in \mathbb{R}+$ controls the amount of signal is retained and. $\sigma_{t} \in \mathbb{R}+$ controls how much noise is added, and $\alpha_{t}$ is modeled as a smooth transition from  $\alpha{1} \sim 1$ to $\alpha_{T} \sim 0$. Following  \cite{kingma2021variational} we define $SNR(t)=\frac{\alpha_{t}^2}{\sigma_{t}^2}$ and use the variance preserving process \cite{sohl2015deep} for which $\alpha_{t}=\sqrt{1-\sigma_{t}^{2}}$.
 
The diffusion process can also be formulated as:
\begin{align}
    & q(z_{t}|z_{s}) = \mathcal{N}(z_t|\alpha_{t|s}z_{s},\sigma_{t|s}^{2}I) \qquad \forall t>s \\
    & \alpha_{t|s} = \alpha_{t}/\alpha_{s} \qquad \sigma_{t|s}^{2} = \sigma_{t}^{2} - \alpha_{t|s}^{2}/\sigma_{s}^{2} \\
    & q(z_{0},z_{1}\hdots,z_{T}|x) = q(z_0|x)\Pi_{t=1}^{T}q(z_{t}|z_{t-1})
\end{align}
And the denoising process can also be written as:
\begin{align}
    & q(z_{s}|x,z_t) = \mathcal{N}(z_s|\mu_{t\rightarrow s} (x,z_{t}),\sigma^{2}_{t\rightarrow s}I) \\
    & \mu_{t\rightarrow s}(x,z_{t})=\frac{\alpha_{t|s}\sigma_{s}^{2}}{\sigma_{t}^{2}}z_{t} + \frac{\alpha_{s}\sigma_{t|s}^{2}}{\sigma_{t}^{2}}x \\
    & \sigma_{t\rightarrow s} = \frac{\sigma_{t|s}\sigma_{s}}{\sigma_{t}}
\end{align}


This true denoising process depends on the data sample $z_{data}$, which is not available when using the model for generating of a new samples. Instead, a neural network $\phi_{\theta}$ is used to approximate the sample $z_{data}$. Specifically, we can reparameterize Equation (1) as $z_{t} = \alpha_{t}z_{data} + \alpha_{t}\epsilon$ with $\epsilon \sim \mathcal{N} (0, I)$ and directly predict the Gaussian noise $\epsilon_{\theta} = \phi_{\theta}(z_{t}, t)$. Thus, $z_{data}$ is simply

The neural network is trained to maximise the likelihood of observed data by optimizing a variational lower bound
on the data, which is equivalent to the simplified training objective \tocite   $\mathcal{L}_{train}= ||\epsilon_{\theta} - \phi_{\theta}(z_{t}, t)||$.

% OTHER:

% As we dont have x we will predict $\hat{x}$ using NN and use it to approximate the true denoising  \\
%  $q(z_{s}|z_{t})=\mathcal{N}(z_{s}|\mu_{t\rightarrow s}(\hat{x} ,z_t),\sigma^{2}_{t\rightarrow s})$.\\
% since the optimisation is easier when predicting the Gaussian noise instead, when the model predict $\hat{\epsilon}_{\theta}(z_t,t)$ that can be used to parameterize the denoising model as $\hat{x}_{\theta}(z_{t},t)=(z_{t}-\sigma_{t}\hat{\epsilon}_{\theta}(z_t,t))\sigma_{t})$.

We use an equivariant GNN to predict the denoising process e.g $\epsilon$

%\subsection{Diffusion process for target-aware  molecule genration }
% In the conditional molecule generation setup, we provide
% fixed three-dimensional context in each step of the denoising process. To this end, we supplement the ligand node point cloud and feature vectors $z^l$ with virtual-receptor nodes and features $z^r$ that remain unchanged throughout the denoising process.
% We parameterize the denoiser predictor as follows $\phi_{\theta}(z^{l}_{t},z^{r}_{data}$
% with an EGNN (\tocite). To process ligand and pocket nodes with a single
% GNN, atom types and residue types are first embedded in
% a joint node embedding space by separate learnable MLPs.
% We use the message-passing scheme from \tocite, however
% we do not update the coordinates of nodes that belong to
% the virtual-receptor to ensure the three-dimensional protein context
% remains fixed throughout the EGNN layers.

%\todo{todo}{subsection}{Insert a rewritten version of Section 3 from our old overleaf.  We should include the sections "Motivation", "Approach", and "Properties of $A_{ij}$".  After that, we should have the sections "Adding in Dihedral Angles", renaming the section of course.  Finally, we should have "Initialization Strategy for the Virtual Receptor" - but only the first part (unless we implement the autoencoder approach, in which case we should include this as well).}


\subsection{Virtual Receptor Atoms}
\paragraph{Motivation}
The driving force behind the creation of the virtual receptor stems from a fundamental desire to enhance the efficiency and effectiveness of molecular generation processes. At its core, the concept revolves around incorporating an encoded representation of the receptor into the generative framework. This strategic move serves a dual purpose: firstly, it seeks to mitigate the computational demands by reducing the need for extensive computations, and secondly, it aims to streamline the representation of the receptor, eliminating redundancies while preserving the crucial graph structure that defines its molecular identity.


\paragraph{Approach} 
To do so we would like to create a sub-graph that is created by a learnable convex sum of the real atoms for the of the receptor that will embedded within the the convex hull that is created by the receptor pocket as follows : 

\begin{equation}
    \tilde{x}_i^r(t) = \sum_{j=1}^M A_{ij}(X^r, t) x_j^r \quad i = 1, \dots, M'
    \label{eq:virtual}
\end{equation}

We refer to $\tilde{x}_i^r(t)$ as the $i^{th}$ virtual receptor atom at diffusion time $t$.  Note that we only generate $M'$ such virtual atoms, where we take $M' \ll M$.  In particular, we suppose that $M' = o(N)$, where $N$ is the number of ligand atoms.

\paragraph{Properties of $A_{ij}$} Returning to Equation (\ref{eq:virtual}), what properties should the functions $A_{ij}$ satisfy?  First, we'll need equivariance with respect to $E(3)$ transformations.  It is easy to see that this will hold if:
\begin{enumerate}
    \item $A_{ij}(\cdot, t)$ is an $E(3)$-invariant function of the set of receptor atoms $X^r$; and
    \item $\sum_{j=1}^M A_{ij}(X^r, t) = 1$ for all $i$.
\end{enumerate}
We will also need $A_{ij}(\cdot, t)$ to be a permutation-invariant function of the set of receptor atoms $X^r$.

\paragraph{Implementation of $A_{ij}$}
We use a version of an EGNN to create an $A_{ij}(\cdot, t)$ that will satisfy our demands as follows.
\begin{equation}
    \breve{h}_j^r = G(h_j^r) \quad j = 1, \dots, M
\end{equation}

\begin{align}
    & q_{jk}^r = Q^r \left( \| x_j^r - x_k^r \|\right) \\
    & b_j \, ,  \bar{b}_j = \texttt{SPLIT} \left( B \left(  \frac{1}{M} \sum_{k=1}^M q_{jk}^r \, \right) \right) \\
    & \bar{b}^{av} = \frac{1}{M} \sum_{j=1}^M \bar{b}_j \quad \quad \bar{g}_j = \bar{G}(h_j) \\
    & \hat{A}_{1j}, \dots, \hat{A}_{M'j} = F\left( \texttt{CONCAT}( b_j ,\bar{g}_j, \bar{b}^{av} , \textcolor{red}{\xi(t=0)} ) \right) \\
    % & A_{ij} = \frac{\hat{A}_{ij}}{\sum_{j'=1}^M \hat{A}_{ij'}} \label{eq:last} 
    & A_{ij} = \frac{e^{\hat{A}_{ij}}}{\sum_{j'=1}^M e^{\hat{A}_{ij'}}}
\end{align}

Where 
\begin{itemize}
    \item $Q$ : a linear layer , followed by a non-linear activation.
    \item $F_i$: concatenate $b_j ,\bar{g}_j, \bar{b}^{av}$  with the Transformer sinusoidal position embedding for the diffusion time $t$ which while training the VR is set to 0.  Then apply a linear layer (mapping a vector to a vector), a non-linear activation, and a linear layer (mapping a vector to a scalar).
    \item $G$: a linear layer , a non-linear activation, and a linear layer .
    \item In the joint EGNN, we will want a way to allow the network to distinguish between ligand and virtual receptor atoms.  The easiest way to do this is to append an extra one-hot of length 2 to the $h$-vectors, where $[1,0]$ indicates ligand and $[0, 1]$ indicates receptor.
\end{itemize}

\paragraph{Initialization}
We propose an learned function for the VR s.t that we learn to VR modules or an encoder-vr and decoder-vr and train to optimize the reconstruction loss like in an auto encoder \tocite model.

The vr-decoding is simple as we only need to replace $M$ with $M'$ e.g learn an $A_(ij)$ functions 

The loss between the original receptor atoms $x_i^r$ and their reconstructions $\breve{x}_i^r$ is a bipartite matching loss, i.e.
    \begin{equation}
        L(X^r, \breve{X}^r) = \min_{\pi \in \mathbb{S}^M} \sum_{i=1}^M \| x_i^r - \tilde{x}_{\pi(i)}^r \|^2
    \end{equation}
where $\pi$ is a permutation, We want the optimization process to be invariant to permutations since we only value the reconstruction on the entire receptor and not the actual indexing of each atom, to do that we use the Hungarian algorithm \tocite to find the best permutation assignment for optimization.

\begin{algorithm}
\caption{Optimize VR Model} \label{alg:cap}
\begin{algorithmic}
% \Require $x\in Data\; \phi - encoder-vr \;  \psi - decoder-vr.$\\
\FOR {$x \in D$}
\State $\tilde{x} = \phi(x,M')$
\newline
\State $x = \psi(x',M)$
\newline
\State loss = $munkres(x,x')$
\newline
\State optimize $\phi$ $\psi$
\ENDFOR{}
\end{algorithmic}
\end{algorithm}



\subsection{Use of Protein Language Embeddings}

The incorporation of Masked Language Model (MLM) models' embeddings has wielded a profound impact across diverse domains \tocite. Specifically, the utilization of ESM (Evolutionary Scale Modeling) \tocite embedding has emerged as promising embedding in for the protein domain, as it has demonstrated its capacity to encapsulate highly informative features for function prediction \tocite and even use it attention map as an proxy for protein structure prediction, relying solely on the sequence data ESM embedding goes beyond the conventional one-hot encoded amino acid representation, offering a richer and more nuanced source of information about the protein's structural characteristics and chemical properties. By leveraging ESM embedding, we augment our ability to inject valuable insights into the protein structure, further enhancing our understanding each amino acid information in the context of it close neighborhood of amino acids and and 3D structre.

We use the ESM embedding from the last layer of the encoder model as the new feature vector for the amino acid node in the graph representing and asign it to the relevant amino-acid by index. 

\todo{todo}{subsection}{Describe the idea, and why it makes sense.  Explain how ESM works.  Show how one can integrate the ESM embeddings in our setting.}

This way we are adding a lot of usefull information to the model about the protein residues chemical information and structural features that affected by it proximal residues, but at the same time we encode the model for an less redundant graph both in nodes number and chemical features in a manner that a keep the compressing fucntion e.g the VR E(3) an permutations equivariant. 

\subsection{Implementation Details} 

We pretrain the VR using the autoencoding method as a preliminary step for the denosier optimization, we initialize the virtual receptor atoms with an Farthest Point Sampling (FPS), which iteratively samples the farthest point and performs distance updating to get an evely sampled points within within the convex hull of the receptor.

We define the receptor as the closest 120 amino acid to the ligand creating and sphere.


\todo{todo}{subsection}{The shell.  Training details.  Anything else?}

==> old/related_work_1.tex <==
\todo{todo}{paragraph}{Diffusion Techniques in General}

\subsection{Denoising Diffusion Probabilistic Models}
Fill

\subsection{Equivariant Graph Neural Networks}
Graph Neural Networks \tocite (GNNs) are learnable functions that composite of Neural network that
process graph-structured data in a permutation-equivariant
way, making them particularly useful for molecular systems
where nodes do not have an intrinsic order. Permutation
invariance means that $GNN(\Pi X) = \Pi GNN(X)$ where
$\Pi$ is an $n \times n$ permutation matrix acting on the node feature
matrix. Since the nodes of the molecular graph represent
the 3D coordinates of atoms, we are interested in additional
equivariance w.r.t. the Euclidean group $E(3)$ or rigid transformations. An E(3)-equivariant GNN (EGNN) satisfies EGNN($\Pi$ X A + b) = $\Pi$ EGNN(X)A + b  where $A \in E(3)$ .


\todo{todo}{paragraph}{Target Aware Molecular Modelling - not diffusion (e.g. autoregressive models, normalizing flows, etc.)}

The research landscape in the field of molecular design has witnessed a dynamic shift, with the emergence of the binding site-conditioned molecular design approach. This novel direction, more recent than the conventional unconditioned molecular design, has opened up exciting avenues for innovation. (Ragoza et al.)is a pioneering work in 2022 stands out as a seminal contribution, employing a conditional Variational Autoencoder (VAE) on a discretized 3D atomic density grid. Following sampling, this grid structure undergoes a transformation into molecular structures through an atom fitting algorithm.

A subsequent class of works, including Drotár et al. (2021), Liu et al. (2022), and Peng et al. (2022), has adopted an autoregressive methodology. Here, the generation of molecular structures unfolds as a sequential process, with the probability distribution of each atom being learned in relation to the preceding atoms. Consequently, molecules are sampled step by step, with each step adding a new segment to the molecule, all within the confines of the binding site.

Luo et al. (2021) introduce a model that captures the likelihood of a particular chemical element occupying a specific point in 3D space. Liu et al. (2022) propose the GraphBP framework, eliminating the need for spatial discretization. Instead, they generate atom types and relative locations while preserving equivariance.

Other notable approaches include recurrent neural networks (RNNs) (Zhang and Chen 2022) And equivariant normalizing flows (Rozenberg)  that holds great promise to both generate new drugs candidates and evaluate the the probability of an suggested drug candidate.

There has been some works about target aware molecules lately that conditioning on the receptor structure () that achieve impressive results.   
\subsection{Target Aware Molecular Modelling}

